Neural-Davidsonian Semantic Proto-role Labeling

We present a model for semantic proto-role labeling (SPRL) using an adapted bidirectional LSTM encoding strategy that we call "Neural-Davidsonian": predicate-argument structure is represented as pairs of hidden states corresponding to predicate and argument head tokens of the input sequence. We demonstrate: (1) state-of-the-art results in SPRL, and (2) that our network naturally shares parameters between attributes, allowing for learning new attribute types with limited added supervision.

==> sections/analysis.tex <==
While we lack the space to perform in-depth analysis on each property, here we select two properties from SPR1 (\textsc{volition} and \textsc{makes physical contact}) and perform a manual error analysis with respect to two systems: \AAAI~\footnote{We obtained the SPR1 dev system predictions of \newcite{teichert2017sprl} via personal communication with the authors.} and \mtSprOne.
For each property, we sample 40 SPR1 dev split instances with gold labels of ``True'' ($>3$) and 40 instances of ``False'' ($\leq 3$), restricted to cases where the two system predictions disagree, i.e. one system made a correct prediction and the other incorrect. We manually label each of these 80 instances for six attributes that may be informative, presented in Table \ref{tab:makes_phys_contact}.

For both properties \mtSprOne~ appears more likely to correctly classify the argument in cases where the predicate is a phrasal verb. This is likely a result of the fact that the BiLSTM has stronger language-modeling capabilities than the \AAAI, particularly with MT pretraining. \mtSprOne~ appears to make more false-positive errors on \textsc{makes physical contact} with pronominal arguments, where \AAAI~ does not. By contrast, for \textsc{volition}, many of the \AAAI~ false positives come from proper nouns or organizations.


==> sections/data.tex <==
\paragraph{SPR1} The SPR1.0 (``SPR1'') dataset introduced by \newcite{TACL674} contains proto-role annotations on 4,912 Wall Street Journal sentences from PropBank \cite{palmer2005_propbank} corresponding to 9,738 predicate-argument pairs with 18 properties each, in total 175,284 property annotations.
All annotations were performed by a single, trusted annotator.
Each annotation is a rating from 1 to 5 indicating the likelihood that the property applies, with an additional ``N/A'' option if the question of whether the property holds is nonsensical in the context.

To compare with prior work \cite{teichert2017sprl}, we treat the SPR1 data as a binary prediction task: the values 4 and 5 are mapped to \textbf{True} (property holds), while the values 1, 2, 3, and ``N/A'' are mapped to \textbf{False} (property does not hold).
In additional experiments, we move to treating SPR1 as a scalar prediction task; in this case, ``N/A'' is mapped to 1, and all other annotation values remain unchanged.

\noindent\textbf{SPR2} The second SPR release \cite{uds2016} contains annotations on 2,758 sentences from the English Web Treebank (EWT) \cite{bies2012english} portion of the Universal Dependencies (v1.2) \cite{silveira14gold}\footnote{We exclude the SPR2 pilot data; if included, the SPR2 release contains annotations for 2,793 sentences.}, corresponding to 6,091 predicate-argument pairs. With 14 proto-role properties each, there are a total of 85,274 annotations, with two-way redundancy. As in SPR1, the value of each annotation is an integral value 1-5 or ``N/A.''
We treat SPR2 as a scalar prediction task, first mapping ``N/A'' to 1, and then averaging the two-way redundant annotation values to a single value.

\paragraph{Word Sense Disambiguation} Aligned with proto-role property annotations in the SPR2 release are word sense disambiguation judgments for the head tokens of arguments. Candidate word senses (fine-grained) from WordNet \cite{fellbaum1998_wordnet} were presented to Mechanical Turk workers (at least three annotators per instance), who selected every applicable sense of the word in the given context. In this work, we map the fine-grained word senses to one of 26 coarse-grained WordNet noun supersenses (e.g., \texttt{noun.animal}, \texttt{noun.event}, \texttt{noun.quantity}, etc.). In many cases, a word may be mapped to more than one supersense. We treat the supersense label on a word as a distribution over supersenses, where the probability assigned to one supersense is proportional to the number of annotators that (indirectly) selected that supersense. In practice, the entropy of these resulting supersense distributions is low, with an average perplexity of 1.42.

\paragraph{PropBank} The PropBank project consists of predicate-argument annotations over corpora for which gold Penn TreeBank-style constituency parses are available.  We use the Unified PropBank release \cite{BONIAL14.1012, ide2017handbook}, which contains annotations over OntoNotes as well as the English Web TreeBank (EWT). Each predicate in each corpus is annotated for word sense, and each argument of each predicate is given a label such as ARG0, ARG1, etc., where the interpretation of the label is defined relative to the word sense.  We use PropBank Frames to map these sense-specific labels to 16 sense-independent labels such as PAG (proto-agent), PPT (proto-patient), etc., and then formulate a task to predict the abstracted labels. Because our model requires knowledge of predicate and argument head words, we ran the Stanford Universal Dependencies converter \cite{SCHUSTER16.779} over the gold constituency parses to obtain Universal Dependency parses, which were then processed by the PredPatt framework \cite{zhang-EtAl:2017:IWCS,uds2016} to identify head words.

\paragraph{English-French Data} The $10^9$ French-English parallel corpus \cite{callisonburch-EtAl:2009:WMT-09} contains 22,520,376 French-English sentence pairs, made up of 811,203,407 French words and 668,412,817 English words.  The corpus was constructed by crawling the websites of international organizations such as the Canadian government, the European Union, and the United Nations.

==> sections/related.tex <==
\todo{Fix, ben moved first part to background} Notably, best models of
\newcite{teichert2017sprl} made use of inter-property factors and
joint training with SRL as an auxiliary task both of which have
parallels in our neural experiments. Subsequent to their work
\cite{white2017inference} used the binary formulation of the task to
create a dataset for exercising models built for Recognizing Textual
Entailment (RTE); this recast version of SPR is most recently used by
\newcite{poliakNAACL18} for semantic evaluation of neural machine
translation models.  \newcite{uds2016} release additional SPR
annotations. We are unaware of other published systems that evaluate
on that data. Using our MT-pretrained, scalar regression architecture
on their train/dev/test splits achieves a Pearson's $\rho$ of 0.577 on
the test set (see Appendix \ref{sec:multi} for related results).
Finally we note prior work on neural models for the parent task of
semantic role labeling (i.e., SRL versus SPRL); in particular,
\newcite{he-EtAl:2017:Long3} also employ bidirectional LSTMs for this
related task.



==> tables/scalar-dev.tex <==
\begin{table}
\begin{center}
\small
\begin{tabular}{llll}
\toprule
{} & \SprOne & \mtSprOne & \SprTwo \\
\midrule
instigation                 &         0.835 &                   0.859 &        0.573 \\
volition                    &         0.869 &                    0.87 &        0.832 \\
awareness                   &          0.87 &                   0.872 &        0.864 \\
sentient                    &         0.895 &                     0.9 &        0.848 \\
physically existed        &         0.814 &                   0.824 &            - \\
existed before              &         0.651 &                   0.666 &        0.601 \\
existed during              &         0.621 &                   0.635 &         0.29 \\
existed after               &         0.562 &                   0.583 &        0.466 \\
created                   &         0.505 &                   0.505 &            - \\
destroyed                 &         0.396 &                   0.403 &            - \\
changed                   &         0.596 &                   0.612 &            - \\
change of state             &         0.611 &                    0.61 &        0.405 \\
change of possession        &         0.558 &                   0.584 &        0.612 \\
change of location          &         0.714 &                   0.724 &        0.507 \\
change of state continuous* &             - &                       - &        0.428 \\
was for benefit*            &             - &                       - &        0.567 \\
stationary                &         0.601 &                   0.611 &            - \\
location                  &         0.526 &                   0.521 &            - \\
physical contact          &          0.74 &                   0.723 &            - \\
manipulated               &          0.73 &                   0.731 &            - \\
was used*                   &             - &                       - &        0.236 \\
partitive*                  &             - &                       - &        0.385 \\
\hline
macro-avg pearson           &         0.717 &                   0.725 &          0.600 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\label{tab:scalar_dev} SPR1 and SPR2 as scalar prediction tasks. Pearson correlation between predicted and gold values.}
\end{table}
